Criteria for Rigor in Visualization Design Study

We develop a new perspective on research conducted through visualization design study that emphasizes design as a method of inquiry and the broad range of knowledge-contributions achieved through it as multiple, subjective, and socially constructed. From this interpretivist position we explore the nature of visualization design study and develop six criteria for rigor. We propose that rigor is established and judged according to the extent to which visualization design study research and its reporting are INFORMED, REFLEXIVE, ABUNDANT, PLAUSIBLE, RESONANT, and TRANSPARENT. This perspective and the criteria were constructed through a four-year engagement with the discourse around rigor and the nature of knowledge in social science, information systems, and design. We suggest methods from cognate disciplines that can support visualization researchers in meeting these criteria during the planning, execution, and reporting of design study. Through a series of deliberately provocative questions, we explore implications of this new perspective for design study research in visualization, concluding that as a discipline, visualization is not yet well positioned to embrace, nurture, and fully benefit from a rigorous, interpretivist approach to design study. The perspective and criteria we present are intended to stimulate dialogue and debate around the nature of visualization design study and the broader underpinnings of the discipline.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> _criteria.PLAUSIBLE.tex <==
\subsection{PLAUSIBLE}
%%\emph{Knowledge claims are reasonable and appropriate.}
\hspace{0.25cm}{\fontfamily{qag}\selectfont\small{\textbf{{
Knowledge claims are reasonable and appropriate. %% OR evidenced and persuasive
}}}}\vspace{1mm}

Plausible knowledge claims made in the context of subjective, interpretivist inquiry must be supported by sufficient and persuasive observations and interpretations. That is, by observations that are representative of the phenomena and processes under study, and by interpretations -- including those that are expressed through a design concept or artifact -- that are congruent with the observations. For example, a data and task abstraction \cite{munzner09} of a domain problem should be grounded in rich evidence that domain experts use, or could benefit from, that representation.
A guideline or other knowledge claim should be developed explicitly from a rich body of evidence, and a visualization system as an effective design should be shown to be grounded in an informed and dynamic design process in which a broad design space was navigated collaboratively. Plausible knowledge claims give others the confidence to use them.

How does a researcher develop an abstracted problem characterization from what she learns from her collaborators and other sources of domain information? How does she design an effective visualization system meant to support a problem that exists in the world? We suggest that the plausibility of \emph{particular} knowledge claims -- \emph{a participant used a visualization in this way} -- is heavily reliant upon a researcher`s use of appropriate design processes and data collection methods, as well as the \say{interpretative construction} \cite{drucker2011humanities} in which she engages. The plausibility of more \emph{general} claims -- \emph{this is a meaningful data and task representation for this problem} -- instead relies on knowledge construction that is reflexive and analytical.

Through a process of \emph{analytic generalization} researchers strive to generalize from specific, situated details into broader, more abstracted concepts \cite{firestone93}. Concepts are constructed as a researcher abstracts from patterns observed in the specifics of a context. In the case of participants in an observed study, Polit \cite{polit10} describes the process as being one where the researcher \say{distinguishes between information that is relevant to all (or many) study participants, in contrast to aspects of the experience that are unique to particular participants... [it] is a matter of identifying evidence that supports that conceptualization.} \cite{polit10}. A predominant method for interpretation and knowledge construction in design study is \emph{reflection}: \say{a process by which experience is brought into consideration . . . to achieve meaning and the capacity to look at things as potentially other than they appear.} \cite{brockbank2003action} The nine-stage framework for conducting design studies emphasizes reflection as a crucial activity \cite{sedlmair12}, but pragmatic guidance in the visualization literature for how and when to reflect is sparse, with many variations in reflective practices and expectations for documentation among design study researchers \cite{2018_cga_reflection}. 

\emph{Memo writing} is an established approach for encouraging and recording reflection in some disciplines. Memos are informal analytic notes that \say{catch your thoughts, capture the comparisons and connections you make, and crystallize questions and directions for you to pursue.} \cite{charmaz2006constructing} Through a (reflexive) conversation-with-self, memo writing can spur new ideas and insights while a researcher engages with her materials and observations. Careful tracking of memos with underlying data can form a rich account of a researcher`s reflective analytic process and reasoning, offering evidence in support of the plausibility of a broad range of knowledge claims. Similarly, explicit recording of design decisions and their justifications through literate visualization supports reflection, interpretation, and analysis while also documenting the process \cite{wood2019design}. 

The more general the knowledge claim, the more abundance is necessary for plausibility. Constructing plausible, general knowledge claims from situated, specific contexts can be achieved through using multiple forms of analysis with a diverse set of rich and reflexive observations. A design study researcher might combine contextual interviews \cite{holtzblatt1993contextual} with a workshop \cite{kerzner2019framework} to establish an initial understanding of a problem domain, using reflective transcriptions \cite{mccurdy2019framework} to interpret the interviews and open-coding to analyze the outputs of the workshop. She might then ideate on possible visualization solutions through rapid prototyping of storyboards \cite{greenberg2011sketching}, refine her ideas based on feedback gathered through speed-dating \cite{hanington2012universal}, and reflexively develop a visualization software artifact using literate visualization \cite{wood2019design}. Through critical reflection on the artifact against the backdrop of existing visualization idioms, she develops a description for a new visualization technique, appropriately scoped to address some, or all of the problem description. 

There is no one way to develop plausible knowledge claims. Design study researchers can, and should be flexible and creative with the methods they employ, while being mindful that the methods and representation practices are coherent with the study's goals and constraints. 


==> _methods.tex <==
\section{Methods}


==> _table.tex <==
%% https://www.tablesgenerator.com/

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}


\begin{table*}[htp]
\caption{Criteria, their rationale, and suggested means for achieving rigorous research through visualization design study.\vspace{0.2cm}}
\label{tab:criteria}
\resizebox{\textwidth}{!}{%

%% Nice font for tables.
\fontfamily{qag}\selectfont

%% \resizebox{\textwidth}{!}{%
\renewcommand{\arraystretch}{1.70}
% {rl}
%% \begin{tabular}{p{0.25\columnwidth}p{0.75\columnwidth}}
\begin{tabular}{p{0.125\textwidth}p{0.875\textwidth}}

\rowcolor[HTML]{EFEFEF} 
\textbf{INFORMED}    & {\small{\textbf{Existing knowledge informs design and facilitates new interpretations.}}} \\
\multicolumn{1}{r}{\textbf{\textit{\small{Important as}}}}
& \textit{\small{Research informed by existing academic and applied knowledge supports interesting and meaningful insights and interpretations.}} \\
\multicolumn{1}{r}{\textbf{\textit{\small{Achievable through}}}} &
\textit{\small{extensive repertoire of design examples; visualization and related domain literature}} \\
%\multicolumn{1}{r}{\textbf{\textit{\small{Informed by}}}} &
%\textit{\small{ADR:theory-engrained artifact, big-tent: rich rigor}} \\

\rowcolor[HTML]{EFEFEF} 
\textbf{REFLEXIVE}   & {\small{\textbf{We effect the research, and it effects us.}}} \\
\multicolumn{1}{r}{\textbf{\textit{\small{Important as}}}}
& \textit{\small{Reflexivity accounts for, and leverages the inherent subjectivity of design study researchers.}} \\
\multicolumn{1}{r}{\textbf{\textit{\small{Achievable through}}}} &
\textit{\small{autoethnography; reflexive diary; critical friends; design critique; formal, structured presentations; peer review}} \\

\rowcolor[HTML]{EFEFEF} 
\textbf{ABUNDANT}    & {\small{\textbf{More is better.}}} \\
\multicolumn{1}{r}{\textbf{\textit{\small{Important as}}}}
& \textit{\small{Abundance provides opportunities to uncover, relate, understand, and justify meaningful insights.}} \\
\multicolumn{1}{r}{\textbf{\textit{\small{Achievable through}}}} &
\textit{\small{saturation; shadow data; thick description; long-term, sustained collaboration; participatory and co-design methods; creative visualization-opportunity workshops; rapid and parallel prototyping; literate visualization}} \\

\rowcolor[HTML]{EFEFEF} 
\textbf{PLAUSIBLE}   & {\small{\textbf{Knowledge claims are reasonable and appropriate.}}} \\
\multicolumn{1}{r}{\textbf{\textit{\small{Important as}}}}
& \textit{\small{Plausible knowledge claims give others the confidence to use them.}} \\
\multicolumn{1}{r}{\textbf{\textit{\small{Achievable through}}}} &
\textit{\small{nested model; reflection; memo writing; literate visualization}} \\

\rowcolor[HTML]{EFEFEF} 
\textbf{RESONANT}    & {\small{\textbf{The research inspires understanding and invites action.}}} \\
\multicolumn{1}{r}{\textbf{\textit{\small{Important as}}}}
& \textit{\small{Resonant research impacts others in the world.}} \\
\multicolumn{1}{r}{\textbf{\textit{\small{Achievable through}}}} &
\textit{\small{thick description; design artifacts that invite engagement; narrated videos, data stories, and annotated imagery; good problems; rich and evocative details of context}} \\

\rowcolor[HTML]{EFEFEF} 
\textbf{TRANSPARENT} & {\small{\textbf{The reporting invites scrutiny.}}} \\
\multicolumn{1}{r}{\textbf{\textit{\small{Important as}}}}
& \textit{\small{Transparent descriptions of activities, processes, evidence and claims allows judgments about the other criteria to be made.}}\\ 
\multicolumn{1}{r}{\textbf{\textit{\small{Achievable through}}}} &
\textit{\small{data and task abstraction with designs; reporting on failures; extensive supplemental materials; findable, annotated evidence base; rich methodological descriptions; audit trail}}

\end{tabular}%
}

\centering\color[HTML]{EFEFEF}\rule{0.8\textwidth}{1pt}

%% \caption{Criteria for Research Through Design Study}
%% \label{tab:criteria}
\end{table*}



==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> template/bibliography.tex <==
\section{Bibliography Instructions}

\begin{itemize}
\item Sort all bibliographic entries alphabetically but the last name of the first author. This \LaTeX/bib\TeX\ template takes care of this sorting automatically.
\item Merge multiple references into one; e.\,g., use \cite{Max:1995:OMF,Kitware:2003} (not \cite{Kitware:2003}\cite{Max:1995:OMF}). Within each set of multiple references, the references should be sorted in ascending order. This \LaTeX/bib\TeX\ template takes care of both the merging and the sorting automatically.
\item Verify all data obtained from digital libraries, even ACM's DL and IEEE Xplore  etc.\ are sometimes wrong or incomplete.
\item Do not trust bibliographic data from other services such as Mendeley.com, Google Scholar, or similar; these are even more likely to be incorrect or incomplete.
\item Articles in journal---items to include:
  \begin{itemize}
  \item author names
	\item title
	\item journal name
	\item year
	\item volume
	\item number
	\item month of publication as variable name (i.\,e., \{jan\} for January, etc.; month ranges using \{jan \#\{/\}\# feb\} or \{jan \#\{-{}-\}\# feb\})
  \end{itemize}
\item use journal names in proper style: correct: ``IEEE Transactions on Visualization and Computer Graphics'', incorrect: ``Visualization and Computer Graphics, IEEE Transactions on''
\item Papers in proceedings---items to include:
  \begin{itemize}
  \item author names
	\item title
	\item abbreviated proceedings name: e.\,g., ``Proc.\textbackslash{} CONF\_ACRONYNM'' without the year; example: ``Proc.\textbackslash{} CHI'', ``Proc.\textbackslash{} 3DUI'', ``Proc.\textbackslash{} Eurographics'', ``Proc.\textbackslash{} EuroVis''
	\item year
	\item publisher
	\item town with country of publisher (the town can be abbreviated for well-known towns such as New York or Berlin)
  \end{itemize}
\item article/paper title convention: refrain from using curly brackets, except for acronyms/proper names/words following dashes/question marks etc.; example:
\begin{itemize}
	\item paper ``Marching Cubes: A High Resolution 3D Surface Construction Algorithm''
	\item should be entered as ``\{M\}arching \{C\}ubes: A High Resolution \{3D\} Surface Construction Algorithm'' or  ``\{M\}arching \{C\}ubes: A high resolution \{3D\} surface construction algorithm''
	\item will be typeset as ``Marching Cubes: A high resolution 3D surface construction algorithm''
\end{itemize}
\item for all entries
\begin{itemize}
	\item DOI can be entered in the DOI field as plain DOI number or as DOI url; alternative: a url in the URL field
	\item provide full page ranges AA-{}-BB
\end{itemize}
\item when citing references, do not use the reference as a sentence object; e.\,g., wrong: ``In \cite{Lorensen:1987:MCA} the authors describe \dots'', correct: ``Lorensen and Cline \cite{Lorensen:1987:MCA} describe \dots''
\end{itemize}


==> template/sections.tex <==
\section{Example Section}

Text \marginpar{\small You can use the margins for comments while editing the submission, but please remove the marginpar comments for submission.} 

Make reference to figures like this (see \autoref{fig:sample}).

\begin{figure}[tb]
 \centering % avoid the use of \begin{center}...\end{center} and use \centering instead (more compact)
 \includegraphics[width=\columnwidth]{paper-count-w-2015-new}
 \caption{A visualization of the 1990--2015 data.
 The image is from \cite{Isenberg:2017:VMC} and is in the public domain.}
 \label{fig:sample}
\end{figure}

\subsubsection{Ejector Seat Reservation}

Text


\paragraph{Confirmed Ejector Seat Reservation}

Text


==> template/style.tex <==
This template is for papers of VGTC-sponsored conferences such as IEEE VIS, IEEE VR, and ISMAR which are published as special issues of TVCG. The template does not contain the respective dates of the conference/journal issue, these will be entered by IEEE as part of the publication production process. Therefore, \textbf{please leave the copyright statement at the bottom-left of this first page untouched}.

\section{Using the Style Template}

\begin{itemize}
\item If you receive compilation errors along the lines of ``\texttt{Package ifpdf Error: Name clash, \textbackslash ifpdf is already defined}'' then please add a new line ``\texttt{\textbackslash let\textbackslash ifpdf\textbackslash relax}'' right after the ``\texttt{\textbackslash documentclass[journal]\{vgtc\}}'' call. Note that your error is due to packages you use that define ``\texttt{\textbackslash ifpdf}'' which is obsolete (the result is that \texttt{\textbackslash ifpdf} is defined twice); these packages should be changed to use ifpdf package instead.
\item Note that each author's affiliations have to be provided in the author footer on the bottom-left corner of the first page. It is permitted to merge two or more people from the same institution as long as they are shown in the same order as in the overall author sequence on the top of the first page. For example, if authors A, B, C, and D are from institutions 1, 2, 1, and 2, respectively, then it is ok to use 2 bullets as follows:
\begin{itemize}
\item A and C are with Institution 1. E-mail: \{a\,$|$\,c\}@i1.com\,.
\item B and D are with Institution 2. E-mail: \{b\,$|$\,d\}@i2.org\,.
\end{itemize}
\item The style uses the hyperref package, thus turns references into internal links. We thus recommend to make use of the ``\texttt{\textbackslash autoref\{reference\}}'' call (instead of ``\texttt{Figure\~{}\textbackslash ref\{reference\}}'' or similar) since ``\texttt{\textbackslash autoref\{reference\}}'' turns the entire reference into an internal link, not just the number. Examples: \autoref{fig:sample} and \autoref{tab:vis_papers}.
\item The style automatically looks for image files with the correct extension (eps for regular \LaTeX; pdf, png, and jpg for pdf\LaTeX), in a set of given subfolders (figures/, pictures/, images/). It is thus sufficient to use ``\texttt{\textbackslash includegraphics\{CypressView\}}'' (instead of ``\texttt{\textbackslash includegraphics\{pictures/CypressView.jpg\}}'').
\item For adding hyperlinks and DOIs to the list of references, you can use ``\texttt{\textbackslash bibliographystyle\{abbrv-doi-hyperref-narrow\}}'' (instead of ``\texttt{\textbackslash bibliographystyle\{abbrv\}}''). It uses the doi and url fields in a bib\TeX\ entry and turns the entire reference into a link, giving priority to the doi. The doi can be entered with or without the ``\texttt{http://dx.doi.org/}'' url part. See the examples in the bib\TeX\ file and the bibliography at the end of this template.\\[1em]
\textbf{Note 1:} occasionally (for some \LaTeX\ distributions) this hyper-linked bib\TeX\ style may lead to \textbf{compilation errors} (``\texttt{pdfendlink ended up in different nesting level ...}'') if a reference entry is broken across two pages (due to a bug in hyperref). In this case make sure you have the latest version of the hyperref package (i.\,e., update your \LaTeX\ installation/packages) or, alternatively, revert back to ``\texttt{\textbackslash bibliographystyle\{abbrv-doi-narrow\}}'' (at the expense of removing hyperlinks from the bibliography) and try ``\texttt{\textbackslash bibliographystyle\{abbrv-doi-hyperref-narrow\}}'' again after some more editing.\\[1em]
\textbf{Note 2:} the ``\texttt{-narrow}'' versions of the bibliography style use the font ``PTSansNarrow-TLF'' for typesetting the DOIs in a compact way. This font needs to be available on your \LaTeX\ system. It is part of the \href{https://www.ctan.org/pkg/paratype}{``paratype'' package}, and many distributions (such as MikTeX) have it automatically installed. If you do not have this package yet and want to use a ``\texttt{-narrow}'' bibliography style then use your \LaTeX\ system's package installer to add it. If this is not possible you can also revert to the respective bibliography styles without the ``\texttt{-narrow}'' in the file name.\\[1em]
DVI-based processes to compile the template apparently cannot handle the different font so, by default, the template file uses the \texttt{abbrv-doi} bibliography style but the compiled PDF shows you the effect of the \texttt{abbrv-doi-hyperref-narrow} style.
\end{itemize}

